The Sample Complexity of Auctions with Side Information

Traditionally, the Bayesian optimal auction design problem has been considered either when the bidder values are i.i.d., or when each bidder is individually identifiable via her value distribution. The latter is a reasonable approach when the bidders can be classified into a few categories, but there are many instances where the classification of bidders is a continuum. For example, the classification of the bidders may be based on their annual income, their propensity to buy an item based on past behavior, or in the case of ad auctions, the click through rate of their ads. We introduce an alternate model that captures this aspect, where bidders are \emph{a priori} identical, but can be distinguished based (only) on some side information the auctioneer obtains at the time of the auction. We extend the sample complexity approach of Dhangwatnotai, Roughgarden, and Yan (2014) and Cole and Roughgarden (2014) to this model and obtain almost matching upper and lower bounds. As an aside, we obtain a revenue monotonicity lemma which may be of independent interest. We also show how to use Empirical Risk Minimization techniques to improve the sample complexity bound of Cole and Roughgarden (2014) for the non-identical but independent value distribution case.

==> rev_monotone_singleagent.tex <==
\subsection{One distribution}
\label{subsec:one_distr}

We first show that revenue monotonicity is true for one distribution:

\begin{lemma}
\textit{Revenue monotonicity} holds when the distribution of only one buyer is replaced.
\end{lemma}

\begin{proof}
We'll write Myerson's optimal auction as an optimization problem. Myerson's auction is the solution to the following program:

	\[
	\begin{array}{lll}
	\textrm{max}    & \sum_{v^{i_1}_1 \in D^1} \dots \sum_{v^{i_n}_n \in D^n} \left( Pr[v^{i_1}_1] \dots Pr[v^{i_n}_n] \right) \left( \sum_{j = 1}^n p_j \left( v^{i_1}_1 \dots v^{i_n}_n \right) \right)  \\
	\textrm{subject to} & u_i \left( v^j_i , v^k_i , t^{-i} \right) = v^j_i x_i(v^k_i, t^{-i}) - p_i \left( v^k_i , t^{-i} \right),  \forall i,v^j_i,v^k_i ,t^{-i}   \\
						& u_i \left( v^j_i , v^j_i , t^{-i} \right) \geq u_i \left( v^j_i , v^k_i , t^{-i} \right),  \forall i,v^j_i,v^k_i, t^{-i}\\
						& u_i \left( v^j_i , v^j_i , t^{-i} \right) \geq 0 , \forall i , v^j_i, t^{-i} \\
	\end{array}
	\]
	
Let $x^*_i , p^*_i$ be the solution for this program, for input distributions $D^1, \dots, D^n$, and $R$ be the value of the objective. We will replace $D^1$ with $\hat{D^1}$ that stochastically dominates it, and use the same allocation rule $x^*_i$ and payment rule $p^*_i$. We can assume, without loss of generality, that the support of the two distributions is the same: if we want to introduce new values in $\hat{D^1}$ we can add them with probability zero in $D_1$. Thus, the difference between $D^1$ and $\hat{D^1}$ is only some swift in probability mass from low to high values. Again, without loss of generality, we can assume that the support of $D^1$ only has two values $l$ and $h > l$, each being realized with some probability $Pr[l]$ and $Pr[h] = 1 - Pr[l]$ respectively. $\hat{D^1}$ assigns some probability $q < Pr[l]$ to $l$.

Thus, the objective can be re-written as:
\begin{multline}
Pr[ l ]  \sum_{v^{i_2}_2 \in D^2} \dots \sum_{v^{i_n}_n \in D^n} \left( Pr[v^{i_2}_2] \dots Pr[v^{i_n}_n] \right) \left( \sum_{j = 1}^n p^*_j \left( l , v^{i_2}_2 \dots v^{i_n}_n \right) \right) + \\ Pr[ h ]  \sum_{v^{i_2}_2 \in D^2} \dots \sum_{v^{i_n}_n \in D^n} \left( Pr[v^{i_2}_2] \dots Pr[v^{i_n}_n] \right) \left( \sum_{j = 1}^n p^*_j \left( h , v^{i_2}_2 \dots v^{i_n}_n \right) \right) \nonumber
\end{multline}

Let's assume that lowering $Pr[l]$ and increasing $Pr[h]$ by some $\epsilon > 0$ strictly decreases the value of the objective. This implies that:

\begin{multline}
\sum_{v^{i_2}_2 \in D^2} \dots \sum_{v^{i_n}_n \in D^n} \left( Pr[v^{i_2}_2] \dots Pr[v^{i_n}_n] \right) \left( \sum_{j = 1}^n p^*_j \left( l , v^{i_2}_2 \dots v^{i_n}_n \right) \right) > \\ \sum_{v^{i_2}_2 \in D^2} \dots \sum_{v^{i_n}_n \in D^n} \left( Pr[v^{i_2}_2] \dots Pr[v^{i_n}_n] \right) \left( \sum_{j = 1}^n p^*_j \left( h , v^{i_2}_2 \dots v^{i_n}_n \right) \right) \nonumber
\end{multline}

This means that we could increase expected revenue by doing the following: set $p^*_j \left( h , v^{i_2}_2 \dots v^{i_n}_n \right) = p^*_j \left( l , v^{i_2}_2 \dots v^{i_n}_n \right)$ and $x^*_j \left( h , v^{i_2}_2 \dots v^{i_n}_n \right) = x^*_j \left( l , v^{i_2}_2 \dots v^{i_n}_n \right) $, for all $j$ and $v^{i_k}_k$. The IC and IR constraints are still satisfied, while the value of the objective strictly increases; a contradiction.
\end{proof}


==> signal_ub_multi.tex <==
\subsubsection{Multiple agents}
\label{subsec:signal_ub_multi}

\zh{In the multiple agent case, buyers' values and signals are also indexed so the current notation is a bit confusing. I propose using $\hat{v}$'s and $\hat{\sigma}$ for samples and $v$'s and $\sigma$'s for actual values and signals of buyers. We can change back if needed.}

% In this Subsection we'll prove Theorem~\ref{thm:onebuyeralg}:

%\anote{add "w.p. at least $1-\delta$"?}
\MultipleAgentUpperBound*

%\bigskip

%Our auction is simply a posted price, at which the bidder can either buy the item or not. The idea is to use the \emph{right} number of signals in the sample that are just below the signal of the bidder. The price posted is simply the best price for the empirical distribution of values corresponding to these signals, guarded against using too few of these values. The entire algorithm is summarized in Algorithm \ref{alg:SingleBuyerSignalUB}.

%\nikhil{Throughout, we need to make sure $k+\ell \leq m$, or define $v_i =\sigma_i =0 $ for all $i>m$.}

\begin{algorithm}[h]
\begin{algorithmic}[1]
%
\STATE \textbf{Samples:~} 
$(\hat{v}_{1}, \hat{\sigma}_{1}), (\hat{v}_{2}, \hat{\sigma}_{2}), \dots, (\hat{u}_{m}, \hat{\sigma}_{m})$, where $\hat{\sigma}_{1} \geq \hat{\sigma}_{2} \geq \dots \geq \hat{\sigma}_{m}$.

\STATE \textbf{Parameter:~}
$\epsilon$

\STATE \textbf{Input:~} 
For each buyer $i$, signal $\sigma_i$ (the value $v_i$ is unobserved); suppose $\hat{\sigma}_{k_i} \geq \sigma_i \geq \hat{\sigma}_{k_i+1}$.

\medskip

\STATE \textbf{Auction:~}\\
%
\STATE Let $\bar{D}^i$ denote the mixture of $D^{\hat{\sigma}_{k_i+1}}, D^{\hat{\sigma}_{k_i+2}}, \dots, D^{\hat{\sigma}_{k_i+\ell}}$; let $\bar{F}^i$ denote the corresponding CDF. 
\STATE For all $i \in [n]$, use $O(\log \frac{n}{\epsilon})$ randomly chosen samples among $\hat{v}_{k_i+1}, \dots, \hat{v}_{k_i+\ell}$ to compute a $2$-approximation of the optimal single-buyer revenue w.r.t.\ $\bar{D}^i$ subject to that sale probability is at least $\frac{1}{2}$ (i.e., $\frac{1}{2} \sr_i \le \max_{p \ge 0 : \bar{F}^i (p) \le \frac{1}{2}} p \big( 1 - \bar{F}^i (p) \big) \le \sr_i$).
\STATE Let $\approxopt = \sum_{i = 1}^{n} \sr_i$.
%\STATE Compute $\approxopt$ using Algorithm \ref{alg:approxopt}.
\STATE Let $V = \{ \frac{8}{\epsilon} \approxopt, \frac{8 (1 - \epsilon)}{\epsilon} \approxopt, \frac{8 (1 - \epsilon)^2}{\epsilon} \approxopt, \dots, \frac{\epsilon}{n} \approxopt, 0 \big\}$.
%\STATE Let there be $m_2 = \Theta(n \epsilon^{-4} \log \frac{n}{\epsilon} \log \frac{1}{\epsilon})$ fresh samples $\vec{v}_1, \dots, \vec{v}_{m_2}$.
\STATE For each buyer $i$, round $\hat{v}_{k_i+1}, \dots, u_{k_i+\ell}$ down to the closest value in $V$;\\ let $\hat{v}^i_1, \dots, \hat{v}^i_\ell$ denote the rounded values; let $E^i$ denote the uniform distribution over $\hat{v}^i_{1}, \dots, \hat{v}^i_{\ell}$.
\STATE Run Myerson auction w.r.t.\ $\mathbf{E} = E^1 \times \dots \times E^n$.
\end{algorithmic}
\caption{$M_{\text{emp}}$, a $1 - O(\epsilon)$ approximately optimal signal auction for multiple agents}
\label{alg:signal_empmyerson}
\end{algorithm}


Similar to the single-buyer case, we divide the realization of all the random variables into 3 stages as follows. 
\begin{enumerate}
\item Sample $m+n$ signals $\sigma^\prime_1, \sigma^\prime_2, \dots, \sigma^\prime_{m+1}$ i.i.d.\ from  $U[0, 1]$.%; suppose $\sigma^\prime_1 \geq \sigma^\prime_2 \ge \dots \ge \sigma^\prime_{m+n}$.
\item Pick a subset of $n$ indices $i_1 \ne \dots \ne i_n \in [m+n]$ uniformly at random and let $\sigma_j = \sigma^\prime_{i_j}$ for all $j \in [n]$; let $\hat{\sigma}_1, \hat{\sigma}_2, \dots, \hat{\sigma}_m$ be the other $m$ signals.
(Note that the  $k_i$ in Algorithm \ref{alg:SingleBuyerSignalUB} is fixed by the end of this stage, and is equal to $j_i-1$.)
\item Sample $m+1$ values, $\hat{v}_j \sim D^{\hat{\sigma}_j}$ for $j \in [m]$ and $v_i \sim \dsigma{i}$ for $i \in [n]$, independently.
\end{enumerate}

%We lower bound the revenue of the auction successively over the randomization in the different stages: first, given the signals $\sigma_1, \sigma_2, \dots, \sigma_m$ and $\sigma$ (Lemma~\ref{lem:onebuyeralg0}), i.e., over the randomness of the third stage, then over the randomness of the last two stages (Lemma~\ref{lem:onebuyeralg1}), and finally over all three stages (Lemma~\ref{lem:onebuyeralg2}). \prettyref{thm:onebuyeralg} then follows from Lemma~\ref{lem:onebuyeralg2} and Definition \ref{def:onebuyeralg3}.
%Assumption~\ref{asm:onebuyeralg3}.

%Let $\hat{D}$ denote the mixed distribution of $\dsigma{k+1}, \dsigma{k+2}, \dots, \dsigma{{k+\ell}}$.
%That is, if we want to draw a value from $\hat{D}$, we first sample $i$ from $\{1, 2, \dots, \ell\}$ uniformly at random, and then draw a value from $\dsigma{k+i}$.

\zh{This should go to the prelim.}
For two distributions $D$ and $D^\prime$, $D \succeq_\epsilon D^\prime$ denote that $D$ $\epsilon$-stochastically dominates $D^\prime$, i.e., for any $v$, $F(v) \le F^\prime(v) + \epsilon$.

%It is easy to verify the following  claims:

Let $\underline{D}^i = D^{\sigma_{k_i+\ell}}$ with CDF $\underline{F}^i$ and $\underline{\vec{D}} = \underline{D}^1 \times \dots \times \underline{D}^n$.

\begin{lemma}
\label{lem:signalmulti_approxopt}
With probability $1 - O(\epsilon)$, $\frac{1}{8} \opt{\underline{\vec{D}}} \le \approxopt \le n \opt{\vec{\bar{D}}}$
\end{lemma}

\begin{proof}
The first inequality holds because $\sr_i \ge \frac{1}{4} \max_{p \ge 0 : \bar{F}^i (p) \le \frac{1}{2}} p \big( 1 - \bar{F}^i (p) \big) \ge \frac{1}{4} \max_{p \ge 0 : \underline{F}^i (p) \le \frac{1}{2}} p \big( 1 - \underline{F}^i (p) \big) \ge \frac{1}{8} \max_{p \ge 0} p \big( 1 - \underline{F}^i (p) \big)$.
The first inequality then follows because $\sum_{i \in [n]} \max_{p \ge 0} p \big( 1 - \underline{F}^i (p) \big) \ge \opt{\underline{\vec{D}}}$.
The second inequality holds because $\sr_i \le \opt{\vec{\bar{D}}}$.
\end{proof}

\begin{lemma}
%\label{claim:onebuyeralg6}
\label{lem:multi_signal_approxopt}
With probability $1 - O(\epsilon)$, we have
%
\[
\opt{\vec{\bar{D}}} \geq \big( 1 - O(\epsilon) \big) \opt{\vec{\underline{D}}} - O(\epsilon) \opt{\vec{D}} \enspace.
\]
%
\end{lemma}

\begin{proof}
By Lemma \ref{lem:multi_signal_approxopt} and Lemma \ref{lem:tailbound}, truncating $\vec{\underline{D}}$ at $\frac{8}{\epsilon} \approxopt$ decreases the optimal revenue by at most at $1 - O(\epsilon)$ factor.
Further, rounding values to the closest power of $1 - \epsilon$ decreases the optimal revenue by at most another $1 - \epsilon$ factor.
Finally, by Lemma \ref{lem:multi_signal_approxopt} rounding all values less than $\frac{\epsilon}{n} \approxopt$ to $0$ decreases the revenue by at most $\epsilon \opt{\vec{\bar{D}}} \le \epsilon \opt{\vec{D}}$.
\end{proof}

As a simple corollary of the above lemma and Theorem \ref{thm:prodconcentrate}, we have the following lemma.

\begin{lemma}
\label{lem:signal_multi_emprev}
%\label{claim:onebuyeralg6}
With probability $1 - O(\epsilon)$, we have
%
\[
\opt{\vec{E}} \geq \big( 1 - O(\epsilon) \big) \opt{\vec{\underline{D}}} - O(\epsilon) \opt{\vec{D}} \enspace.
\]
\end{lemma}

\zh{What we need here is an approximate version of revenue monotonicity for distributions that satisfy approximately stochastically domination.}

The following claim is a simple application of Chernoff-Hoeffding bound.
\begin{claim}
\label{claim:multi_approx_dominance}
$D^{\sigma_i} \succeq \bar{D}^i \succeq_\delta E^i$ for $\delta = \frac{\epsilon^2}{n^2}$.
\end{claim}

\begin{lemma}
%	\label{lem:onebuyeralg0}
%
\[
\E \big[ \rev{M_{\emp}}{\vec{D}} | \sigma_1, \dots, \sigma_m, \sigma \big] \geq \big( 1 - O(\epsilon) \big) \opt{\vec{\underline{D}}} - O(\epsilon) \opt{\vec{D}} \enspace.
\]
\end{lemma}
\begin{proof}	%[Proof of Lemma \ref{lem:onebuyeralg0}]
By Claim \ref{claim:multi_approx_dominance}, for all $i \in [n$] there exists a distribution $\tilde{D}^i \succeq E^i$ such that the total variation distance between $D^i$ and $D^{\sigma_i}$ is at most $\delta = \frac{\epsilon^2}{n^2}$. 
Thus, we have that (a) $\vec{\tilde{D}} \succeq \vec{E}$ and (b) the total variation distance between $\vec{D}$ and $\vec{\tilde{D}}$ is at most $n\delta = \frac{\epsilon^2}{n}$.
By (a) and Theorem \ref{thm:revenueMonotonicity} we get that $\rev{M_{\emp}}{\vec{\tilde{D}}} \ge \rev{M_{\emp}}{\vec{E}} = \opt{\vec{E}}$.
By (b) and that maximum revenue per run is at most $\frac{8}{\epsilon} \approxopt \le \frac{8n}{\epsilon} \opt{\vec{D}}$ (Lemma \ref{lem:signalmulti_approxopt}), we get that $\rev{M_{\emp}}{\vec{D}} \ge \rev{M_{\emp}}{\vec{\tilde{D}}} - O(\epsilon) \opt{\vec{D}}$.
Putting together with Lemma \ref{lem:signal_multi_emprev} proves the lemma.
\end{proof}

%\nikhil{Notation needs to be changed from hereon.}

Next, we lower bound the revenue of the above auction over the randomness of the last two stages:

\begin{lemma}
%\label{lem:onebuyeralg1}
\begin{equation}
%\label{eqn:onebuyeralg1}
\E \big[ \opt{\vec{\underline{D}}} | \sigma^\prime_1, \dots, \sigma^\prime_{m+n} \big] \geq \big( 1 - O(\epsilon) \big) \frac{1}{{m+n \choose n}} \sum_{\{i_1, \dots, i_n\} \subset [m+n]} \opt{D^{\sigma^\prime_{i_1}} \times \dots \times D^{\sigma^\prime_{i_n}}}
\end{equation}
\end{lemma}

\begin{lemma}
%\label{lem:onebuyeralg1}
\begin{equation}
%\label{eqn:onebuyeralg1}
\E \big[ \opt{\vec{D}} | \sigma^\prime_1, \dots, \sigma^\prime_{m+n} \big] = \frac{1}{{m+n \choose n}} \sum_{\{i_1, \dots, i_n\} \subset [m+n]} \opt{D^{\sigma^\prime_{i_1}} \times \dots \times D^{\sigma^\prime_{i_n}}}
\end{equation}
\end{lemma}

%Finally, we will lower bound the revenue of the above auction over the randomness of all three stages.

%\begin{lemma}
%\label{lem:onebuyeralg2}
%\anote{add "w.p. at least $1-\delta$"?}
%\[
%\E \big[ \rev{M_\emp}{D^\sigma} \big] \geq (1 - \epsilon)^2 \int_0^{1 - \frac{\ell}{m+1}} \opt{D^\sigma} d\sigma
%\]
%\end{lemma}
%\nikhil{Should the upper limit on the  integral be $1- \frac \ell {m+1}$? } 
%\begin{proof}

%\end{proof}




\begin{proof}[Proof of Theorem \ref{thm:multibuyeralg}]
\end{proof}
